VisFly-Lab: Unified Differentiable Framework for First-Order Reinforcement Learning of Quadrotor Control

First-order reinforcement learning with differentiable simulation is promising for quadrotor control, but practical progress remains fragmented across task-specific settings. To support more systematic development and evaluation, we present a unified differentiable framework for multi-task quadrotor control. The framework is wrapped, extensible, and equipped with deployment-oriented dynamics, providing a common interface across four representative tasks: hovering, tracking, landing, and racing. We also present the suite of first-order learning algorithms, where we identify two practical bottlenecks of standard first-order training: limited state coverage caused by horizon initialization and gradient bias caused by partially non-differentiable rewards. To address these issues, we propose Amended Backpropagation Through Time (ABPT), which combines differentiable rollout optimization, a value-based auxiliary objective, and visited-state initialization to improve training robustness. Experimental results show that ABPT yields the clearest gains in tasks with partially non-differentiable rewards, while remaining competitive in fully differentiable settings. We further provide proof-of-concept real-world deployments showing initial transferability of policies learned in the proposed framework beyond simulation.

==> horizon_length.tex <==
\label{sec:h_analysis}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/h_analysis.png}
    \caption{Training curves for hovering and landing tasks with different horizon lengths. Performance is evaluated with horizons of 16, 32, 64, 96, and 128.}
    \label{fig:h_analysis}
\end{figure}

The optimal horizon length in SHAC is typically reported as 32, but the results obtained in this work reveal a different trend. As shown in \reffig{fig:h_analysis}, for the hovering task the algorithm achieves comparable final returns with horizons of 64, 96, and 128. This discrepancy can be attributed to the increased complexity of the quadrotor dynamics discussed in \refsec{sec:dynamics}. In contrast, for the landing task the set of effective horizons narrows to a single value, 96, suggesting that not only the underlying dynamics but also the task context play a crucial role in determining suitable hyperparameters.




==> introduction.tex <==
Learning-based quadrotor control is attractive because it can amortize computation into a fast policy and avoid solving online optimization at deployment time. Among these approaches, first-order reinforcement learning (RL) with differentiable simulation is especially appealing for quadrotors because their dynamics are smooth and analytically tractable in simulation.

% Differentiable simulation has recently opened a new avenue for policy learning.
Instead of relying purely on sampled policy-gradient estimates such as those used in maximizing expected return \cite{haarnoja2018soft} and likelihood \cite{schulman2017proximal}, first-order RL optimize policies by backpropagating analytical gradients through differentiable dynamics. Such methods have shown strong promise in continuous control \cite{xu_accelerated_2022, n_wiedemann_training_2023}, and quadrotors are among the most suitable platforms for this paradigm due to their smooth dynamics.

Despite this promise, practical progress on first-order learning for quadrotor control remains limited. Existing differentiable-quadrotor studies are still mostly task-specific, making it difficult to compare training behavior across tasks under a shared interface and dynamics model. 
In addition, practical first-order training raises two recurring issues: horizon-based rollouts may under-cover feasible initial states, and reward designs with binary or conditional components can reduce the usefulness of purely differentiable rollout objectives. Specifically, when part of the reward is non-differentiable, backpropagation-through-time only propagates gradients through the differentiable reward terms, which introduces gradient bias with respect to the full task objective.

This paper addresses both issues. We develop a unified differentiable framework for multi-task quadrotor control, with deployment-oriented dynamics, differentiable simulation, and a common interface for four representative tasks: hovering, tracking, landing, and racing. 
% Within this setting, we identify two practical bottlenecks of standard first-order training: limited state coverage from horizon initialization and degraded learning under partially non-differentiable rewards. 
Within this setting, we identify two practical bottlenecks of standard first-order training: limited state coverage from horizon beginning and degraded learning under partially non-differentiable rewards.
To address them, we propose \emph{Amended Backpropagation Through Time} (ABPT), a first-order actor-critic method that combines short-horizon differentiable optimization, a value-based auxiliary objective, and visited-state initialization.
We evaluate the proposed framework and method on the four tasks and compare ABPT against the widely-used baselines. Results show that ABPT improves convergence and final performance. We also provide proof-of-concept real-world deployments showing initial transferability beyond simulation.
The main contributions of this paper are as follows:
\begin{itemize}
    \item We develop a unified differentiable framework for multi-task quadrotor control that is wrapped, extensible, and directly supports downstream development of first-order RL methods.
    \item We identify two practical bottlenecks of standard first-order learning in this setting: limited state coverage from horizon initialization and gradient bias caused by partially non-differentiable rewards.
    \item We propose Amended Backpropagation Through Time (ABPT), which combines differentiable rollout optimization, a value-based auxiliary objective, and visited-state initialization to mitigate gradient bias and improve training across representative quadrotor tasks.
    \item We demonstrate through simulation experiments that ABPT outperforms strong baselines across representative tasks, and we provide proof-of-concept real-world deployments showing initial transferability.
\end{itemize}

==> introduction2.tex <==
Learning-based quadrotor control is attractive because it can amortize computation into a fast policy and thereby avoid expensive online optimization during deployment. Among these approaches, first-order reinforcement learning (RL) with differentiable simulation is particularly appealing for quadrotors, since their dynamics are smooth, structured, and largely governed by physical laws that can be modeled analytically in simulation. Instead of relying purely on sampled policy-gradient estimates, first-order methods can exploit analytical gradients through differentiable dynamics, offering a promising route toward more efficient policy optimization in continuous-control settings [1]–[4]. Quadrotors are among the most suitable robotic platforms for this paradigm due to their well-understood dynamics and the availability of compact yet expressive simulation models.

Despite this promise, practical progress on first-order learning for quadrotor control remains limited. Existing differentiable-quadrotor studies have primarily treated analytical gradients as a tool for solving specific tasks, such as hovering, tracking, adaptation, or obstacle avoidance, rather than organizing training and evaluation under a shared and reusable setting. As a result, it remains difficult to compare optimization behavior across tasks, reward structures, and algorithmic variants under a common interface and dynamics model. Moreover, several existing studies rely on simplified kinematic assumptions rather than deployment-oriented dynamics, introducing an additional mismatch between training and deployment beyond the standard sim-to-real gap.

These limitations motivate the need for a unified and deployment-oriented testbed for first-order RL of quadrotor control. Such a framework should support multiple representative tasks under shared interfaces, while incorporating sufficiently realistic differentiable dynamics to better reflect practical deployment constraints. A unified setting is valuable not only for downstream method development, but also for exposing how first-order optimization behaves under different reward structures and task characteristics. In particular, moving from fully differentiable objectives to tasks that include binary or conditional reward terms can significantly change the training behavior of gradient-based methods, and such effects are difficult to study systematically without a common benchmark and implementation pipeline.

Within such a unified setting, we observe two recurring practical difficulties in standard first-order training. First, horizon-based rollout training may under-cover feasible initial states, since many implementations initialize a new rollout horizon from the terminal state of the previous one, leaving part of the dynamically feasible state space insufficiently explored during optimization. Second, when task rewards are partially non-differentiable, backpropagation-through-time can only propagate gradients through the differentiable reward terms, introducing a gradient bias with respect to the full task objective. This issue is particularly relevant in quadrotor tasks such as landing and racing, where binary or conditional success-related rewards play an important behavioral role but do not directly contribute gradients through differentiable rollouts.

To study and address these issues, this paper develops a unified differentiable framework for multi-task quadrotor control. The framework is wrapped, extensible, and directly supports downstream development of first-order RL methods. It provides deployment-oriented differentiable dynamics together with a common interface across four representative quadrotor tasks: hovering, tracking, landing, and racing. These tasks span different levels of control difficulty and reward differentiability, making the framework suitable both for controlled empirical analysis and for developing more robust first-order learning pipelines. On top of this framework, we propose Amended Backpropagation Through Time (ABPT), a first-order actor-critic method that combines short-horizon differentiable optimization, a value-based auxiliary objective, and visited-state initialization. The purpose of ABPT is to amend standard differentiable rollout training in the presence of the above bottlenecks, especially the gradient bias caused by partially non-differentiable rewards.

We evaluate the proposed framework and ABPT on the four representative tasks and compare ABPT against representative baseline methods. The results show that ABPT is competitive across the unified benchmark and yields the clearest gains in tasks with partially non-differentiable rewards, while remaining effective in fully differentiable settings. In addition, we provide proof-of-concept real-world deployments of policies learned in the proposed framework, offering initial evidence of deployability and transferability beyond simulation rather than a comprehensive quantitative hardware benchmark. This positioning is consistent with the intended role of the hardware experiments in this work: to demonstrate initial sim-to-real feasibility of the proposed framework and learning pipeline, rather than superiority over alternative deployment pipelines.

The main contributions of this paper are summarized as follows:

We develop a unified, wrapped, and extensible differentiable framework for multi-task quadrotor control, with deployment-oriented dynamics and a shared interface across hovering, tracking, landing, and racing.

Using this framework, we identify two practical bottlenecks of standard first-order learning in this setting: limited state coverage caused by horizon initialization and gradient bias caused by partially non-differentiable rewards.

We propose ABPT, which combines differentiable rollout optimization, a value-based auxiliary objective, and visited-state initialization to mitigate these issues and improve training robustness across representative quadrotor tasks.

We demonstrate through simulation experiments that ABPT is competitive across the unified benchmark and particularly beneficial in partially non-differentiable tasks, and we provide proof-of-concept real-world deployments showing initial transferability of the learned policies beyond simulation.

==> learning_rate_robustness.tex <==
\label{sec:learning_rate_robustness}


%In our experiments, learning rate could even be set as 0.01, which is an intolerant number that will cause training instability for most of deep learning. 
We evaluated the training performance using different learning rates. The fully differentiable hovering task is used for evaluation.
As shown in \reffig{fig:precise}, the proposed ABPT exhibits stable and fast
training performance in all learning rates. PPO has the highest variance compared to other FOG-based algorithms, as expected demonstrating that FOG is much more precise than ZOG. 
%As a common sense, the larger learning rate is, the more probably updates might "overshoot", resulting to training oscillations. 
Increasing the learning rate yields a slight improvement on acceleration once it surpasses 0.001 for PPO and SHAC, while ABPT's convergence speed stably grows with increasing learning rate. 

==> limitation.tex <==
\label{sec:limitation}
\li{
ABPT enhances the efficiency and robustness of training processes utilizing analytical gradients, even in scenarios involving partially differentiable reward structures.
However, while it significantly mitigates the gradient bias caused by non-differentiable reward components, it may still fail to fully eliminate extreme bias if the biased gradient is excessively large.
% In other words, if the non-differentiable rewards contribute too heavily to the overall reward, ABPT's training performance may also degrade. 
Therefore, when designing reward functions, priority should be given to incorporating smooth and differentiable variables to the greatest extent possible. In the following work, we will further explore how to adaptively mix the gradient while avoiding incurring excessive computation for mixture-ratio estimation.
% However, while it significantly mitigates the gradient bias arising from non-differentiable reward components, if the biased gradient is absolutely opposite from actual optimization direction, it sometimes fails to entirely eliminate such extreme bias. Therefore, we strongly recommend that, when designing reward functions, priority should be given to incorporating smooth and differentiable variables to the greatest extent possible. This approach ensures more stable and reliable optimization during training. In the following work, we will further explore how to adaptively mix the gradient while avoiding cost too much resources on mixture ratio computation.
%好像没讲清楚，而且显得本方法还有很大缺陷，不如不提
}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> proof.tex <==
\label{sec:proof}
We now prove that ABPT's objective function mitigates gradient bias by combining value gradients with first-order gradients. This theoretical analysis shows how our approach maintains accurate gradient directions despite non-differentiable rewards.

Suppose the value function $Q_\phi$ is well trained, the accumulated reward within the horizon can be approximated as: 
 \begin{equation}
 \small
     \mathcal{G}_\theta^{t:t+N} \approx\mathcal{V}_{\theta|\phi}^{t}-(1-d)\gamma^N \mathcal{V}_{\theta|\phi}^{t+N+1}.
 \end{equation}
 Its value gradient is then given by 
 \begin{equation}
 \small
     \nabla_\theta^{[q]} \mathcal{G}_\theta^{t:t+N} = \nabla_\theta\mathcal{V}_{\theta|\phi}^{t} - (1-d)\gamma^N  \nabla_\theta \mathcal{V}_{\theta|\phi}^{t+N+1}
 \end{equation}
regardless of the differentiability of the rewards. Noting that, unlike \cite{xu_accelerated_2022},  we specifically use action-value function $Q_\phi$ to compute the value to ensure $\mathcal{G}_\theta^{t:t+N}$ is differentiable with respect to $\theta$, which makes this derivative expression meaningful, otherwise the derivative would be zero if using $V_\phi$ solely with state input. Let $\nabla_\theta\mathcal{G}_\theta^{t:t+N}$ denote the first-order gradient of the accumulated reward. The average of the two gradients can be expressed as:
\begin{equation}
\small
\bar{\nabla}_\theta \mathcal{G}_\theta^{t:t+N} = \frac{1}{2}\left(\nabla^{[q]}_\theta \mathcal{G}_\theta^{t:t+N} + \nabla_\theta \mathcal{G}_\theta^{t:t+N}\right).
\end{equation}
It is straightforward to verify that taking the derivative of \refeqn{eq:loss_actor} yields the following gradient for backpropagation:


\begin{equation} 
\label{eq:combined_gradients}
\small
\begin{aligned}
& \nabla_\theta \mathcal{J}_\theta = \frac{1}{|\mathcal{B}|}\sum_{i=1}^{|\mathcal{B}|}\left[ \bar{\nabla}_\theta \mathcal{G}_\theta^{t:t+N+}+(1-d)\gamma^N \nabla_\theta \mathcal{V}_{\theta|\phi}^{t+N+1} \right] \\
& = \frac{1}{2|\mathcal{B}|}\sum_{i=1}^{|\mathcal{B}|} \left[\underbrace{\nabla^{[q]}_\theta \mathcal{G}_\theta^{t:t+N}}_{\nabla\mathcal{J}^{0}_\theta} + \underbrace{\nabla_\theta \mathcal{G}_\theta^{t:t+N}+(1-d)\gamma^N \nabla_\theta \mathcal{V}_{\theta|\phi}^{t+N+1}}_{\nabla\mathcal{J}^N_\theta} \right].
\end{aligned}
\end{equation}

Therefore, the difference between this gradient and the gradient (\ref{eq:first_order_n_return}) used in \cite{xu_accelerated_2022}  is that the first-order gradients in \refeqn{eq:first_order_n_return} are combined with the value gradients. By leveraging this combination, our method remains effective in guiding the parameter updates toward the correct direction, when the first-order gradient is biased due to the non-differentiable rewards.

We conduct a simple experiment to assess the effectiveness of incorporating the 0-step return in addressing gradient bias. We deliberately detach parts of rewards in the hovering task (see \refsec{sec:taskDefine}) to mimic non-differentiable rewards, then backpropagate to compute gradient of network parameter. As shown in \reffig{fig:detach_diff}, combining the 0-step return with the N-step return in the objective function \refeqn{eq:loss_actor} for training significantly reduces the model parameter residuals.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/detach_diff.png}
    \caption{ The curve shows the difference between the parameters trained with fully differentiable and partially differentiable rewards. We deliberately detach parts of the rewards to interrupt gradient backpropagation and retrain the policy with or without combining the 0-step return. }
    \label{fig:detach_diff}
\end{figure}

==> relatedWork.tex <==
\subsection{Reinforcement Learning}

Traditional reinforcement learning can be divided into two classes: model-free RL and model-based RL.
Model-free RL includes value-based and policy-gradient methods. Value-based methods learn value functions to estimate long-term rewards. DQN \cite{mnih2013playing} introduced neural networks for discrete actions, while DDPG \cite{lillicrap2015continuous} extended this to continuous action spaces. TD3 \cite{fujimoto2018addressing} reduced overestimation bias with multiple value networks, and SAC \cite{haarnoja2018soft} used a maximum entropy framework for robust high-dimensional learning. Policy-gradient methods directly optimize policies using gradients. TRPO \cite{schulman2015trust} stabilized updates via trust regions, and PPO \cite{schulman2017proximal} simplified optimization with a clipped surrogate objective.

In contrast to model-free RL which treats the environment as a black box, model-based RL \cite{moerland_model-based_2023} introduces an additional process to learn the environment's dynamics. %Its approaches are highly varied. 
For example, PILCO~\cite{deisenroth2011pilco} and Dyna-Q~\cite{sutton1990integrated} leveraged  learned environment models to generate simulated experiences to accelerate training. Methods like \cite{chua2018deep,watter2015embed} employ trajectory sampling to plan over learned environment models. Dreamer \cite{hafner_dream_2019} embedded entire functions into a latent space, enabling end-to-end policy updates via backpropagation-through-time (BPTT). Despite their advantages, existing RL methods do not explicitly utilize the dynamics of robotics that can be precisely described by physical laws. 
 

%Model-free RL algorithms are the most widely used to train intelligent policies across interdisciplinary fields. They can be further divided into two categories : value-based methods and policy-gradient methods. Value-based methods focus on learning value functions to estimated expected long-term rewards. DQN \cite{mnih2013playing} achieved significant success in playing Atari by introducing neural networks to estimate long-term values. To adapt to more realistic continuous action spaces, DDPG \cite{lillicrap2015continuous} replaced the discrete action probabilities with continuous action outputs directly from the actor network. TD3 \cite{fujimoto2018addressing} introduced multiple value networks to mitigate the issue of overestimation bias and improve stability. SAC \cite{haarnoja2018soft} incorporated a maximum entropy framework to enhance exploration by balancing exploitation and exploration, enabling robust learning for high-dimensional tasks. Policy-gradient methods directly optimize the policy parameters by using stochastic gradients or the zero-order gradients derived from the rewards. TRPO \cite{schulman2015trust} improved training stability by constraining the magnitude of policy updates to stay within a "trust region."
%PPO \cite{schulman2017proximal} further simplified the optimization process by introducing a clipped surrogate objective, striking a balance between exploration and stability while maintaining computational efficiency.

%In contrast to model-free RL which treats the environment as a black box, model-based RL \cite{moerland_model-based_2023} introduces an additional process to learn the environment's dynamics. %Its approaches are highly varied. 
%For example, PILCO~\cite{deisenroth2011pilco} and Dyna-Q~\cite{sutton1990integrated} leveraged  learned environment models to generate simulated experiences to accelerate training. Methods like \cite{chua2018deep,watter2015embed} employ trajectory sampling to plan over learned environment models. Dreamer \cite{hafner_dream_2019} embedded entire functions into a latent space, enabling end-to-end policy updates via backpropgation through time (BPTT). Despite their advantages, model-based RL disregards the potential advantages of exploiting known environment privileges, such as explicitly utilizing the transition function in robotics, whose dynamics can be precisely described by physical laws. 


\subsection{Differentiable Simulators}
Policy learning via differentiable physics is an approach that integrates the physical simulations with differentiable dynamics to enable policy learning directly by using gradient-based optimization. Making the dynamics differentiable in the simulator is the key to this approach. 
%Differentiable simulations provide effective tools for research in FOG-based optimization. 
DiffTaichi \cite{hu_difftaichi_2020} is a comprehensive differentiable physics engine that includes simulations of fluid, gas, rigid body movement, and more. 
In the field of robotics, Brax \cite{freeman_brax_2021} offers differentiable versions of common RL benchmarks, built on four physics engines, including JAX and MuJoCo \cite{todorov_mujoco_2012}. Another line of research focuses on addressing challenges in contact-rich environments. For example, Heiden et al. \cite{heiden_neuralsim_2021} tackle the contact-rich discontinuity problem in quadruped robots by employing a neural network to approximate the residuals. Dojo \cite{howell_dojo_2023} enhances contact solvers and integrates various integrators to accelerate computations while maintaining fidelity. %Other research efforts focus on improving decision-making capabilities rather than control policies. 这两个区别么？也没有引文
VisFly \cite{li_visfly_2024} introduces a versatile drone simulator with fast rendering, based on Habitat-Sim \cite{savva2019habitat}, providing a platform for high-level applications. To enhance the efficiency, many simulators leverage GPU-accelerated frameworks like JAX \cite{schoenholz_jax_2020} and PyTorch \cite{paszke2017automatic} for faster computations.

 \subsection{First-order Gradient Training}
 With the differentiable simulators, the policy can be trained through BPTT by using the first-order gradients. Though first-order gradients enable faster and more accurate gradient computation, they suffer from gradient explosion/vanishing or instability caused by smooth dynamics. Many attempts have tried to address these issues and strengthen robustness. PODS \cite{mora_pods_2021} leverages both first- and second-order gradients with respect to cumulative rewards. SHAC \cite{xu_accelerated_2022} employs an actor-critic framework, truncates the learning window to avoid vanishing/exploding gradients, and smooths the gradient updates. AOBG \cite{suh_differentiable_2022} combines ZOG (policy gradient) with FOG, using an adaptive ratio based on gradient variance in the minibatch to avoid the high variance typical of pure FOG in discontinuous dynamics. AGPO \cite{gao_adaptive_gradient_2024} replaces ZOG in mixture with critic predictions, as Q-values offer lower empirical variance during policy rollouts. While both AGPO and AOBG converge to ultimate rewards in significantly fewer timesteps, the mixture ratio requires excessive computational resources, leading to longer wall-time.  AHAC \cite{georgiev2024adaptivehorizonactorcriticpolicy} makes the horizon adaptive to reduce sampling error in scenarios involving stiff dynamics.
 SAPO \cite{xing2024stabilizing} introduces entropy to strengthen the training stability especially in soft-body simulation.

 




==> sac_exp.tex <==
\label{sec:sac}

  SAC is typically used as a baseline for value-iteration model-free algorithms and has shown strong performance across various simulation benchmarks. However, in real-world scenarios—particularly for planning six-dimensional motions in free space—the size and variance of the observation space are much greater than in simulation. This increased complexity makes it significantly more difficult to train the critic. Since the degree of critic undertraining is critical for value-iteration methods like SAC but less so for policy-iteration methods, PPO has become the most widely used algorithm for training policies deployed in practice.

To validate SAC’s performance, we include it only in the hovering task as \reffig{fig:sac} . The results show that, in real-world applications, SAC performs much worse than PPO. Therefore, in the experiments presented in this paper, we focus our comparisons on PPO.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/std_compa_forSAC.png}
    \caption{Training curves of hovering for baselines including SAC.}
    \label{fig:sac}
\end{figure}

==> tables/bptt_paras.tex <==
\begin{table*}[h!]
\scriptsize
\centering
\caption{Hyperparameters of BPTT}
\label{tab:comparision}
\begin{tabular}{l | l | l | l | l}
\toprule
& \textbf{Hovering} & \textbf{Tracking} & \textbf{Landing} & \textbf{Racing} \\
\midrule
learning rate $\alpha$ & 0.01 & 0.01 & 0.005 & 0.002  \\
number of parallel environments $n$ & 100 & 100 & 100 & 100  \\
discount factor $\gamma$ & 0.99 & 0.99 & 0.99 & 0.99  \\
weight decay & 0.00001 & 0.00001  & 0.00001 & 0.00001 \\ 
decay learning rate & False & False & False & True \\ 
horizon length $H$ & 256 & 256 & 256 & 512 \\
Optimizer & Adam & Adam & Adam & Adam  \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/mtd_ablation.tex <==

\begin{table*}[h!]
\scriptsize
\centering
\caption{Hyperparameters of ABPT no 0-step Value}
\label{tab:comparision}
\begin{tabular}{l |  l | l | l | l}
\toprule
& \textbf{Hovering} & \textbf{Tracking} & \textbf{Landing} & \textbf{Racing} \\
\midrule
learning rate $\alpha$ & 0.01 & 0.01 & 0.01 & 0.01  \\
number of parallel environments $n$ & 100 & 100 & 100 & 100  \\
discount factor $\gamma$ & 0.99 & 0.99 & 0.99 & 0.99  \\
training critic steps per minibatch & 10 & 10 & 10 & 10 \\ 
weight decay & 0.00001 & 0.00001  & 0.00001 & 0.00001 \\ 
target critic update factor $\tau$ & 0.005 & 0.005 & 0.005 & 0.005 \\ 
decay learning rate & False & True & False & True \\ 
value estimation factor $\lambda$  & 0.95 &  0.95 &  0.95 &  0.95 \\
horizon length $H$ & 96 & 96 & 96 & 96 \\
replay buffer size & 1000000 & 1000000 & 1000000 & 50000 \\
Optimizer & Adam & Adam & Adam & Adam  \\
\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[ht!]
\scriptsize
\centering
\caption{Hyperparameters of ABPT no Entropy}
\label{tab:comparision}
\begin{tabular}{l |  l | l | l | l}
\toprule
& \textbf{Hovering} & \textbf{Tracking} & \textbf{Landing} & \textbf{Racing} \\
\midrule
learning rate $\alpha$ & 0.01 & 0.01 & 0.002 & 0.002  \\
number of parallel environments $n$ & 100 & 100 & 100 & 100  \\
discount factor $\gamma$ & 0.99 & 0.99 & 0.99 & 0.99  \\
training critic steps per minibatch & 10 & 10 & 10 & 10 \\ 
weight decay  & 0.00001 & 0.00001 & 0.00001 & 0.00001 \\ 
target critic update factor $\tau$ & 0.005 & 0.005 & 0.005 & 0.005 \\ 
decay learning rate  & False & True & False & True \\ 
value estimation factor $\lambda$ &  0.95 &  0.95 &  0.95 &  0.95 \\
horizon length $H$ & 96 & 96 & 96 & 96 \\
replay buffer size  & 1000000& 1000000 & 1000000 & 50000 \\
Optimizer & Adam & Adam & Adam & Adam  \\

\bottomrule
\end{tabular}

\end{table*}

.

\begin{table*}[ht!]
\scriptsize
\centering
\caption{Hyperparameters of ABPT no 0-step Value no Entropy}
\label{tab:comparision}
\begin{tabular}{l |  l | l | l | l}
\toprule
& \textbf{Hovering} & \textbf{Tracking} & \textbf{Landing} & \textbf{Racing} \\
\midrule
learning rate $\alpha$ & 0.01 & 0.01 & 0.002 & 0.002  \\
number of parallel environments $n$ & 100 & 100 & 100 & 100  \\
discount factor $\gamma$ & 0.99 & 0.99 & 0.99 & 0.99  \\
training critic steps per minibatch & 10 & 10 & 10 & 10 \\ 
weight decay  & 0.00001 & 0.00001 & 0.00001 & 0.00001 \\ 
target critic update factor $\tau$ & 0.005 & 0.005 & 0.005 & 0.005 \\ 
decay learning rate  & False & True & False & True \\ 
value estimation factor $\lambda$ &  0.95 &  0.95 &  0.95 &  0.95 \\
horizon length $H$ & 96 & 96 & 96 & 96 \\
replay buffer size  & 1000000& 1000000 & 1000000 & 50000 \\
Optimizer & Adam & Adam & Adam & Adam  \\

\bottomrule
\end{tabular}

\end{table*}



==> tables/mtd_paras.tex <==

\begin{table*}[h!]
\scriptsize
\centering
\caption{Hyperparameters of ABPT}
\label{tab:comparision}
\begin{tabular}{l |  l | l | l | l}
\toprule
& \textbf{Hovering} & \textbf{Tracking} & \textbf{Landing} & \textbf{Racing} \\
\midrule
learning rate $\alpha$ & 0.01 & 0.01 & 0.01 & 0.01  \\
number of parallel environments $n$ & 100 & 100 & 100 & 100  \\
discount factor $\gamma$ & 0.99 & 0.99 & 0.99 & 0.99  \\
training critic steps per minibatch & 10 & 10 & 10 & 10 \\ 
weight decay & 0.00001 & 0.00001  & 0.00001 & 0.00001 \\ 
target critic update factor $\tau$ & 0.005 & 0.005 & 0.005 & 0.005 \\ 
decay learning rate & False & True & False & True \\ 
value estimation factor $\lambda$  & 0.95 &  0.95 &  0.95 &  0.95 \\
horizon length $H$ & 96 & 96 & 96 & 96 \\
replay buffer size & 1000000 & 1000000 & 1000000 & 50000 \\
Optimizer & Adam & Adam & Adam & Adam  \\

\bottomrule
\end{tabular}

\end{table*}



==> tables/ppo_paras.tex <==
\begin{table*}[!h]
\scriptsize
\centering
\caption{Hyperparameters of PPO}
\label{tab:comparision}
\begin{tabular}{l |  l | l | l | l}
\toprule
& \textbf{Hovering} & \textbf{Tracking} & \textbf{Landing} & \textbf{Racing} \\
\midrule
learning rate $\alpha$ & 0.001 & 0.0002 & 0.0005 & 0.001  \\
number of parallel environments $n$ & 100 & 100 & 100 & 100  \\
discount factor $\gamma$ & 0.99 & 0.99 & 0.99 & 0.99  \\
minibatch size & 25600 & 25600 & 25600 & 51200  \\
training critic steps per minibatch & 5 & 5 & 5 & 5 \\ 
weight decay & 0.00001 & 0.00001  & 0.00001 & 0.00001 \\ 
GAE $\lambda$ & 1 & 1 & 1 & 1  \\
Optimizer & Adam & Adam & Adam & Adam  \\
\bottomrule
\end{tabular}
\end{table*}



==> tables/r_robust.tex <==
\begin{table*}[ht!]
\scriptsize
\centering
\caption{Hyperparameters of ABPT upon Velocity-based Reward in Racing }
\label{tab:comparision}
\begin{tabular}{l |  l | l |  l | l}
\toprule
  & \textbf{ABPT}& \textbf{SHAC}& \textbf{BPTT}& \textbf{PPO} \\
\midrule
learning rate $\alpha$  & 0.02 & 0.02   & 0.002 & 0.0002 \\
number of parallel environments $n$ & 100 & 100 & 100 & 100  \\
discount factor $\gamma$  & 0.99 & 0.99 & 0.99 & 0.99  \\
training critic steps per minibatch  & 10  & 10 & 10 & 5\\ 
weight decay  & 0.00001  & 0.00001 & 0.00001 & 0.00001 \\ 
target critic update factor $\tau$  & 0.005& 0.005& - &- \\ 
decay learning rate  & True  & True  & True & -\\ 
value estimation factor $\lambda$  &  0.95   &  0.95 & -&-\\
horizon length $H$& 96 & 96 & 512 & -\\
replay buffer size  & 50000 &- &- &- \\
minibatch size & - & - & - & 51200  \\
GAE  &- &- &- & 1 \\
Optimizer & Adam & Adam & Adam & Adam  \\

\bottomrule
\end{tabular}

\end{table*}

==> tables/shac_paras.tex <==

\begin{table*}[ht!]
\scriptsize
\centering
\caption{Hyperparameters of SHAC}
\label{tab:comparision}
\begin{tabular}{l |  l | l | l | l}
\toprule
& \textbf{Hovering} & \textbf{Tracking} & \textbf{Landing} & \textbf{Racing} \\
\midrule
learning rate $\alpha$ & 0.01 & 0.01 & 0.01 & 0.002  \\
number of parallel environments $n$ & 100 & 100 & 100 & 100  \\
discount factor $\gamma$ & 0.99 & 0.99 & 0.99 & 0.99  \\
training critic steps per minibatch & 10 & 10 & 10 & 10 \\ 
weight decay & 0.00001 & 0.00001  & 0.00001 & 0.00001 \\ 
target critic update factor $\tau$ & 0.005 & 0.005 & 0.005 & 0.005 \\ 
decay learning rate & False & False & False & True \\ 
value estimation factor $\lambda$  & 0.95 &  0.95 &  0.95 &  0.95 \\
horizon length $H$ & 96 & 96 & 96 & 96 \\
Optimizer & Adam & Adam & Adam & Adam  \\
\bottomrule
\end{tabular}

\end{table*}



==> training_paras.tex <==
\label{sec:para}

Tables 2$\sim$5 contain the parameters for the baseline experiments, Tables 6$\sim$8 for the ablation experiments, and Table 9 for the reward robustness experiments. Noting that, Simulators like dm\_control often ignore the complexity of real-world dynamics. In our case, we conducted detailed system identification and matched our simulation to actual quadrotor behavior, including communication delay, motor dynamics, aerodynamic drag, PID control, thrust modeling, and time synchronization. (see VisFly). This complexity makes optimal hyperparameters differ from original baselines.
\input{tables/shac_paras}
\input{tables/ppo_paras}
\input{tables/bptt_paras}
\input{tables/mtd_paras}
\input{tables/mtd_ablation}
\input{tables/r_robust}
